3DGS-ReLoc: 3D Gaussian Splatting for Map Representation and Visual ReLocalization

This paper presents a novel system designed for 3D mapping and visual relocalization using 3D Gaussian Splatting. Our proposed method uses LiDAR and camera data to create accurate and visually plausible representations of the environment. By leveraging LiDAR data to initiate the training of the 3D Gaussian Splatting map, our system constructs maps that are both detailed and geometrically accurate. To mitigate excessive GPU memory usage and facilitate rapid spatial queries, we employ a combination of a 2D voxel map and a KD-tree. This preparation makes our method well-suited for visual localization tasks, enabling efficient identification of correspondences between the query image and the rendered image from the Gaussian Splatting map via normalized cross-correlation (NCC). Additionally, we refine the camera pose of the query image using feature-based matching and the Perspective-n-Point (PnP) technique. The effectiveness, adaptability, and precision of our system are demonstrated through extensive evaluation on the KITTI360 dataset.

==> figures/ape_map.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3in]{images/live_loc/ape_map0.png}\\
{\scriptsize(a) Absolute Pose Error Map of Seq 0}\\
\includegraphics[width=3in]{images/live_loc/ape_map1.png}\\
{\scriptsize(b) Absolute Pose Error Map of Seq 1}\\
\end{tabular} 
\label{fig:init_loc_y}
\end{figure}

==> figures/init_loc_x.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3.3in]{images/init_loc/x_nnc.png}\\
{\scriptsize(a) X Error-Normalized Cross Correlation}\\
\includegraphics[width=3.3in]{images/init_loc/query_x.png}\\
{\scriptsize(b) Query Image}\\
\includegraphics[width=3.3in]{images/init_loc/best_x.png}\\
{\scriptsize(c) Best Matched Rendered Image Along X}\\
\includegraphics[width=3.3in]{images/init_loc/worst_x.png}\\
{\scriptsize(d) Worst Matched Rendered Image Along X}\\
\end{tabular} 
\caption{Evaluation of Initial Localization with Respect to Translation Error} 
\label{fig:init_loc_x}
\end{figure}

==> figures/init_loc_y.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3.3in]{images/init_loc/yaw_nnc.png}\\
{\scriptsize(a) Yaw Error-Normalized Cross Correlation}\\
\includegraphics[width=3.3in]{images/init_loc/query_y.png}\\
{\scriptsize(b) Query Image}\\
\includegraphics[width=3.3in]{images/init_loc/best_y.png}\\
{\scriptsize(c) Best Matched Rendered Image Along Yaw}\\
\includegraphics[width=3.3in]{images/init_loc/worst_y.png}\\
{\scriptsize(d) Worst Matched Rendered Image Along Yaw}\\
\end{tabular} 
\caption{Evaluation of Initial Localization with Respect to Rotation Error} 
\label{fig:init_loc_y}
\end{figure}

==> figures/light_change.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3in]{images/lighting/gt1.png}\\
{\scriptsize(a) Ground with Reflection}\\
\includegraphics[width=3in]{images/lighting/gt0.png}\\
{\scriptsize(a) Ground without Reflection after Moving forward}\\
\includegraphics[width=3in]{images/lighting/rendering.png}\\
{\scriptsize(c) Rendered Image}\\
\end{tabular} 
\label{fig:light_change}
\end{figure}
